PHANGS-JWST First Results: The Influence of Stellar Clusters on PAHs in Nearby Galaxies

We present a comparison of theoretical predictions of dust continuum and polycyclic aromatic hydrocarbon (PAH) emission with new JWST observations in three nearby galaxies: NGC 628, NGC 1365, and NGC 7496. Our analysis focuses on a total of 1063 compact stellar clusters and 2654 stellar associations previously characterized by HST in the three galaxies. We find that the distributions and trends in the observed PAH-focused infrared colors generally agree with theoretical expectations, and that the bulk of the observations is more aligned with models of larger, ionized PAHs. These JWST data usher in a new era of probing interstellar dust and studying how the intense radiation fields near stellar clusters and associations play a role in shaping the physical properties of PAHs.

==> tables/table.tex <==
NGC7793      &0.95&0.1& 0.0&3.77$\pm$0.12&0.05$\pm$0.03&-2.00$\pm$0.01&2.67$\pm$0.58& 0.08$\pm$0.24&-0.53$\pm$0.03& 6.98$\pm$0.17& 9.38$\pm$0.05\\
